Embedded error estimation and adaptive step-size control for optimal explicit strong stability preserving Runge--Kutta methods

We construct a family of embedded pairs for optimal strong stability preserving explicit Runge-Kutta methods of order $2 \leq p \leq 4$ to be used to obtain numerical solution of spatially discretized hyperbolic PDEs. In this construction, the goals include non-defective methods, large region of absolute stability, and optimal error measurement as defined in [5,19]. The new family of embedded pairs offer the ability for strong stability preserving (SSP) methods to adapt by varying the step-size based on the local error estimation while maintaining their inherent nonlinear stability properties. Through several numerical experiments, we assess the overall effectiveness in terms of precision versus work while also taking into consideration accuracy and stability.

==> Makefile <==
BUILDIR= build-dir
BIB = bibtex
PROJECT = embedded_ssp_methods
PLATFORM = $(shell uname)
IMEXFILES := $(wildcard sidafa/*.tex)

# files to include in the tar file
ListOfFiles := $(PROJECT).tex $(PROJECT).bib $(PROJECT).bbl figs Makefile

ifeq ($(PLATFORM),Linux)
	VIEWER = gnome-open
	TEX = pdflatex --interaction=batchmode #-output-directory=$(BUILDIR)
else
	VIEWER = open
	TEX = pdflatex --interaction=batchmode #-output-directory=$(BUILDIR)
endif

.PHONY = all view clean build

build : $(PROJECT).tex $(IMEXFILES)
	$(TEX) $(PROJECT).tex
	$(BIB) $(PROJECT)
	$(BIB) $(PROJECT)
	$(TEX) $(PROJECT).tex
	$(BIB) $(PROJECT)
	$(TEX) $(PROJECT).tex
	$(TEX) $(PROJECT).tex


changeNaN : ssp_tables/*.tex
	for f in ssp_tables/*tex; do \
		sed -i .bak 's:NaN:--:g' $$f; \
	done

view : $(PROJECT).pdf
	$(VIEWER) $< 

packup : build clean
	@tar -zcf $(PROJECT).tar.gz $(ListOfFiles)

clean:
	rm -f *.{aux,log,blg,out,toc,lof,lot,pdf}

